Dynamics and Stability of Non-Smooth Dynamical Systems with Two Switches

One of the most common hypotheses on the theory of non-smooth dynamical systems is a regular surface as switching manifold, at which case there is at least well-defined and established Filippov dynamics. However, systems with singular switching manifolds still lack such well-established dynamics, although present in many relevant models of phenomena where multiple switches or multiple abrupt changes occur. At this work, we leverage a methodology that, through blow-ups and singular perturbation, allows the extension of Filippov dynamics to the singular case. Specifically, tridimensional systems whose switching manifold consists of an algebraic manifold with transversal self-intersection are considered. This configuration, known as double discontinuity, represents systems with two switches and whose singular part consists of a straight line, where ordinary Filippov dynamics is not directly applicable. For the general, non-linear case, beyond defining the so-called fundamental dynamics over the singular part, general theorems on its qualitative behavior are provided. For the affine case, however, theorems fully describing the fundamental dynamics are obtained. Finally, this fine-grained control over the dynamics is leveraged to derive Peixoto like theorems characterizing semi-local structural stability.

==> sec/framework/sub/blowup.tex <==
\subsection{Blow-up}%
\label{sec:framework:sub:blowup}

The first step consists in applying a polar blow-up at the origin of the slice
represented at \cref{sec:framework:sub:blowup:subfig:slice} or, in other words,
a \textbf{cylindrical blow-up} at $\Sigma_{x}$. See
\cref{sec:framework:sub:blowup:subfig:slice_blowup}.  More specifically,
assuming that the components of $\mathbf{F} \in \mathcal{D}_3^k$ can be written as

\begin{equation*}
  \mathbf{F}_i = (w_i, p_i, q_i),
\end{equation*}

\noindent we apply the blow-up $\phi_1: \mathbb{R} \times S^1 \times \mathbb{R}^+ \to \mathbb{R}^3$ given by

\begin{equation*}
  \phi_1(x,\theta,r) = (x, r\cos{\theta}, r\sin{\theta}),
\end{equation*}

\noindent which induces a piecewise smooth vector field $\mathbf{\tilde{F}} =
  [(\phi_1)_*^{-1}\mathbf{F}] \circ \phi_1$ whose components are given by

\begin{equation*}
  \mathbf{\tilde{F}}_i =
  \left(w_i,
  \frac{q_i \cos{\theta} - p_i \sin{\theta}}{r},
  p_i \cos{\theta} + q_i \sin{\theta} \right),
\end{equation*}

\noindent where $w_i$, $p_i$ and $q_i$ must be calculated at the point
$\phi_1(x,\theta,r)$. We then define the set

\begin{equation*}
  \tilde{\mathcal{D}}_3^k =
  \left\{\mathbf{\tilde{F}} = [(\phi_1)_*^{-1}\mathbf{F}] \circ \phi_1 ;~
  \mathbf{F} \in \mathcal{D}_3^k
  \right\}
\end{equation*}

\noindent of all blow-up induced vector fields.

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\linewidth}
    \def\svgwidth{\linewidth}
    \import{tex/sec/framework/fig/}{slice_blowup.pdf_tex}
    \caption{Blow-up.}%
    \label{sec:framework:sub:blowup:subfig:slice_blowup}
  \end{subfigure}
  \qquad
  \begin{subfigure}[b]{0.45\linewidth}
    \def\svgwidth{\linewidth}
    \import{tex/sec/framework/fig/}{slice_regul.pdf_tex}
    \caption{Regularization.}%
    \label{sec:framework:sub:blowup:subfig:slice_regul}
  \end{subfigure}
  \caption{Framework process.}%
  \label{sec:framework:sub:blowup:fig:framework_process}
\end{figure}

An extremely important observation at this point is the fact that, according
to~\cite[p.~498]{Llibre2015}, the induced vector field $\mathbf{\tilde{F}}$ has
only \textbf{regular discontinuities}, i.e., classical Filippov theory, as
presented at \cref{sec:preliminaries}, is sufficient for its study. More
precisely, we have now a piecewise smooth vector field $\mathbf{\tilde{F}}$
given by the four smooth vector fields $\mathbf{\tilde{F}}_i$, which induces the
four \textbf{slow-fast systems}

\begin{equation}
  \label{sec:framework:sub:blowup:eq:slow-fast}
  \left\{\begin{matrix*}[l]
    \dot{x} = w_i\\
    r \dot{\theta} = q_i \cos{\theta} - p_i \sin{\theta}\\
    \dot{r} = p_i \cos{\theta} + q_i \sin{\theta}
  \end{matrix*}\right.,
\end{equation}

\noindent where $\dot{\square} = \sfrac{d\square}/{dt}$; $w_i$, $p_i$ and $q_i$
must be calculated at the point $\phi_1(x,\theta,r)$; and $r$ is the time
rescaling factor.

The study of the dynamics of~\eqref{sec:problem:eq:piecewise_field} has
therefore been reduced to the study of the slow-fast systems
\eqref{sec:framework:sub:blowup:eq:slow-fast}. In particular, the dynamics over
$\Sigma_x$, previously undefined, can now be associated with
\cref{sec:framework:sub:blowup:eq:slow-fast} at $r = 0$, which is given by the
combination of the dynamics of the \textbf{reduced system}

\begin{equation}
  \label{sec:framework:blowup:eq:slow_system}
  \left\{\begin{matrix*}[l]
    \dot{x} = w_i\\
    0 = q_i \cos{\theta} - p_i \sin{\theta}\\
    \dot{r} = p_i \cos{\theta} + q_i \sin{\theta}
  \end{matrix*}\right.
\end{equation}

\noindent and the dynamics of the \textbf{layer system}

\begin{equation}
  \label{sec:framework:blowup:eq:fast_system}
  \left\{\begin{matrix*}[l]
    x' = 0\\
    \theta' = q_i \cos{\theta} - p_i \sin{\theta}\\
    r' = 0
  \end{matrix*}\right.,
\end{equation}

\noindent where $\square' = \sfrac{d\square}/{d\tau}$ with $t = r \tau$; and the
components $w_i$, $p_i$ and $q_i$ must be calculated at the point
$\phi_1(x,\theta,0) = (x,0,0)$.

More geometrically, the dynamics over $\Sigma_{x}$ in
\cref{sec:problem:eq:piecewise_field} can now be associated to the dynamics over
the cylinder $C = \mathbb{R} \times S^1$ divided in the four infinite stripes

\begin{align*}
   & S_2 = \mathbb{R} \times [\sfrac{\pi}{2}, \pi],
   & S_1                                             & = \mathbb{R} \times [0,\sfrac{\pi}{2}],      \\
   & S_3 = \mathbb{R} \times [\pi, \sfrac{3\pi}{2}],
   & S_4                                             & = \mathbb{R} \times [\sfrac{3\pi}{2}, 2\pi],
\end{align*}

\noindent as represented at \cref{sec:framework:sec:blowup:fig:stripes}, where
acts the slow-fast systems given by
\cref{sec:framework:blowup:eq:slow_system,sec:framework:blowup:eq:fast_system},
respectively. As we previously said, according to \cite[p.~498]{Llibre2015}, the
four lines where these stripes intersect has regular discontinuities at most.
Finally, the analysis of the dynamics over each stripe $S_i$ can then be carried
out as presented in \cref{sec:preliminaries:sub:gsp:exmp:regul_process}.

\begin{figure}[ht]
  \centering
  \def\svgwidth{0.95\linewidth}
  \import{tex/sec/framework/fig/}{stripes.pdf_tex}
  \caption{Green cylinder $C$ divided in the four stripes $S_i$. A scheme of
    the stripe $S_1$ is also put in evidence.}
  \label{sec:framework:sec:blowup:fig:stripes}
\end{figure}

In particular, the first two equations of the system
\eqref{sec:framework:blowup:eq:slow_system} are independent of $r$ and,
therefore, it can be decoupled as

\begin{equation}
  \label{sec:framework:blowup:eq:slow_system_cyl}
  \left\{\begin{matrix*}[l]
    \dot{x} = w_i\\
    0 = q_i \cos{\theta} - p_i \sin{\theta}\\
  \end{matrix*}\right.,
\end{equation}

\noindent which gives the \textbf{reduced dynamics} over $S_i$; and

\begin{equation}
  \label{sec:framework:blowup:eq:slow_system_rad}
  \dot{r} = p_i \cos{\theta} + q_i \sin{\theta},
\end{equation}

\noindent which gives the respective \textbf{slow radial dynamics} or, in other
words, it indicates how the external dynamics communicates with the dynamics
\eqref{sec:framework:blowup:eq:slow_system_cyl} over the cylinder: entering
($\dot{r} > 0$), leaving ($\dot{r} < 0$) or staying ($\dot{r} = 0$) at $S_i$.

Analogously, the first two equations of the system
\eqref{sec:framework:blowup:eq:fast_system} are independent of $r$ and,
therefore, it can also be decoupled as

\begin{equation}
  \label{sec:framework:blowup:eq:fast_system_cyl}
  \left\{\begin{matrix*}[l]
    x' = 0\\
    \theta' = q_i \cos{\theta} - p_i \sin{\theta}
  \end{matrix*}\right.,
\end{equation}

\noindent which gives the \textbf{layer dynamics} over $S_i$; and

\begin{equation}
  \label{sec:framework:blowup:eq:fast_system_rad}
  r' = 0,
\end{equation}

\noindent which gives the respective \textbf{fast radial dynamics} over the
cylinder.

Summarizing, we conclude that the dynamics over $\Sigma_x$ behaves as described
in the theorem below, whose proof consists in the analysis done above.

\begin{thm}[Double Discontinuity Dynamics]
  \label{sec:framework:blowup:thm:dynamics}
  Given $\mathbf{F} \in \mathcal{D}_3^k$ with components $\mathbf{F}_i = (w_i,
    p_i, q_i)$, let $\mathbf{\tilde{F}} \in \tilde{\mathcal{D}}_3^k$ be the
  induced vector field by the blow-up $\phi_1(x,\theta,r) = (x, r\cos{\theta},
    r\sin{\theta})$. Then, this blow-up associates the dynamics over $\Sigma_x$
  with the following dynamics over the cylinder $C = \mathbb{R} \times S^1 =
    S_1 \cup \ldots \cup S_4$: over each stripe $S_i$ acts a slow-fast dynamics
  whose reduced dynamics is given by

  \begin{equation}
    \label{sec:framework:blowup:thm:dynamics:eq:reduced}
    \left\{\begin{matrix*}[l]
      \dot{x} = w_i\\
      0 = q_i \cos{\theta} - p_i \sin{\theta}\\
    \end{matrix*}\right.,
  \end{equation}

  \noindent with slow radial dynamics $\dot{r} = p_i \cos{\theta} + q_i
    \sin{\theta}$; and layer dynamics given by

  \begin{equation}
    \label{sec:framework:blowup:thm:dynamics:eq:layer}
    \left\{\begin{matrix*}[l]
      x' = 0\\
      \theta' = q_i \cos{\theta} - p_i \sin{\theta}
    \end{matrix*}\right.,
  \end{equation}

  \noindent with fast radial dynamics $r' = 0$. Finally, at every equation above
  the functions $w_i$, $p_i$ and $q_i$ must be calculated at the point
  $\phi_1(x,\theta,0) = (x,0,0)$. \qed
\end{thm}

In order to perform a deeper analysis of the dynamics given by
\cref{sec:framework:blowup:thm:dynamics} with GSP-Theory as described at
\cref{sec:preliminaries:sub:gsp}, let $S_i$ be one of the cylinder's stripe and
let

\begin{equation*}
  \mathcal{M}_i = \left\{ (x, \theta) \in \mathbb{R} \times S^1 ;~
  f_i(x, \theta, 0) = 0 \right\}
\end{equation*}

\noindent be its slow manifold, where $f_i(x, \theta, 0) = q_i \cos{\theta} -
  p_i \sin{\theta}$.

Given $(x_0, \theta_0, 0) \in \mathcal{M}_i \times \left\{ 0 \right\}$, the
Jacobian matrix of the complete layer system
\cref{sec:framework:blowup:eq:fast_system} over this point is

\begin{equation*}
  \mathbf{J}_{\text{fast}} =
  \begin{bmatrix}
    0       & 0              & 0 \\
    (f_i)_x & (f_i)_{\theta} & 0 \\
    0       & 0              & 0
  \end{bmatrix},
\end{equation*}

\noindent where $(f_i)_x$ and $(f_i)_{\theta}$ represents the partial
derivatives calculated at $\left( x_0, \theta_0, 0 \right)$. The eigenvalues of
this matrix are the elements of the set $\left\{0, 0, (f_i)_{\theta} \right\}$
and, therefore, $(x_0, \theta_0)$ is normally hyperbolic if, and only if,
$(f_i)_{\theta} \neq 0$. However, we observe that, since we are over the slow
manifold, then $(f_i)_{\theta} = 0$ leads to the homogeneous linear system

\begin{equation*}
  \left\{\begin{matrix*}[r]
    f_i = 0 \\
    (f_i)_{\theta} = 0
  \end{matrix*}\right.
  \quad \sim \quad
  \left\{\begin{matrix}
    q_i \cos{\theta} - p_i \sin{\theta} = 0 \\
    q_i \sin{\theta} + p_i \cos{\theta} = 0
  \end{matrix}\right.
  \quad \sim \quad
  \begin{bmatrix}
    \cos{\theta} & -\sin{\theta} \\
    \sin{\theta} & \cos{\theta}
  \end{bmatrix}
  \begin{bmatrix}
    q_i \\
    p_i
  \end{bmatrix}
  =
  \begin{bmatrix}
    0 \\
    0
  \end{bmatrix},
\end{equation*}

\noindent whose only solution is the trivial, $p_i = q_i = 0$, since the
trigonometrical matrix above is invertible ($\text{det} \equiv 1$) for every
$\theta \in S^1$ and, therefore, we conclude that $(f_i)_{\theta} \neq 0$
whenever

\begin{equation}
  \tag{WFH}
  \label{sec:framework:sub:blowup:eq:weak_fund_hypo}
  p_i \neq 0 \quad \text{or} \quad q_i \neq 0,
\end{equation}

\noindent henceforth, called \textbf{weak fundamental hypothesis}, or WFH for
short. We also observe that

\begin{equation*}
  (f_i)_x = (q_i)_x \cos{\theta} - (p_i)_x \sin{\theta}
\end{equation*}

\noindent which, as above, supposing $(f_i)_x = 0$ leads to the homogeneous
linear system

\begin{equation*}
  \left\{\begin{matrix*}[r]
    q_i \cos{\theta} - p_i \sin{\theta} = 0 \\
    (q_i)_x \cos{\theta} - (p_i)_x \sin{\theta} = 0
  \end{matrix*}\right.
  \quad \sim \quad
  \begin{bmatrix*}[c]
    q_i     & p_i     \\
    (q_i)_x & (p_i)_x
  \end{bmatrix*}
  \begin{bmatrix}
    \cos{\theta} \\
    \sin{\theta}
  \end{bmatrix}
  =
  \begin{bmatrix}
    0 \\
    0
  \end{bmatrix}
\end{equation*}

\noindent which only admits the absurd solution $\cos{\theta} = \sin{\theta} =
  0$ if the matrix above is invertible. Hence, we can ensure $(f_i)_x \neq 0$ by
imposing this absurd, i.e.,

\begin{equation}
  \tag{SFH}
  \label{sec:framework:sub:blowup:eq:strong_fund_hypo}
  0 \neq
  \det{\begin{bmatrix*}[c]
      q_i     & p_i     \\
      (q_i)_x & (p_i)_x
    \end{bmatrix*}}
  =
  q_i (p_i)_x - p_i (q_i)_x
\end{equation}

\noindent which always implies the weak fundamental hypothesis and, therefore,
will be called \textbf{strong fundamental hypothesis}, or SFH for short.

\begin{cor}
  \label{sec:framework:sub:blowup:cor:radial_dynamics}
  The radial dynamics can only be transversal ($\dot{r} \neq 0$)  to the
  cylinder $C$ over the slow manifold $\mathcal{M}_i$. More over, under WFH, it
  is in fact transversal.
\end{cor}

\begin{proof}
  The first part of the statement is assured by
  \cref{sec:framework:blowup:thm:dynamics}. For the second part, just observe
  that $\dot{r} = - (f_i)_{\theta} \neq 0$ under WFH.
\end{proof}

\begin{cor}
  \label{sec:framework:sub:blowup:cor:explicit_slow_manifold}
  The slow manifold $\mathcal{M}_i$ is locally a graph $\left( x, \theta(x)
    \right)$ under WFH. However, if $\norm{(f_i)_{\theta}}$ admits a global
  positive minimum, then $\mathcal{M}_i$ is globally a graph $\left( x,
    \theta(x) \right)$. Either way, $\theta(x)$ is of class $C^k$.
\end{cor}

\begin{proof}
  The first part is assured by the usual Implicit Function Theorem applied to
  $f_i(x_0, \theta_0, 0) = 0$ over $\mathcal{M}_i$, since under WFH we have
  $\norm{(f_i)_{\theta}} > 0$. Analogously, the second part is assured by the
  Global Implicit Function Theorem found in \cite[p.~253]{Zhang2006}, which
  requires a stronger hypothesis.
\end{proof}

\begin{cor}
  \label{sec:framework:sub:blowup:cor:normal_hyperbolic}
  The slow manifold $\mathcal{M}_i$ is normally hyperbolic at every point that
  satisfies the WFH.
\end{cor}

\begin{proof}
  Just observe that the only non-trivial eigenvalue, $(f_i)_{\theta}$, is
  non-zero under the WFH.
\end{proof}

\begin{cor}
  \label{sec:framework:sub:blowup:cor:singularities}
  The hyperbolic singularities of the reduced system
  \cref{sec:framework:blowup:thm:dynamics:eq:reduced} acts as hyperbolic saddle
  or node singularities of $S_i$ under WFH.
\end{cor}

\begin{proof}
  Let $\mathbf{P} = \left( x_0, \theta_0 \right) \in \mathcal{M}_i$ be a
  hyperbolic singularity of the reduced system, i.e., $w_i(x_0, 0, 0) = 0$ with
  eigenvalue $\lambda_1 = (w_i)_{x}(x_0, 0, 0) \neq 0$. We have two
  possibilities:

  \begin{itemize}
    \item $\lambda_1 > 0 \Rightarrow (j^s, j^u) = (0,1)$; or
    \item $\lambda_1 < 0 \Rightarrow (j^s, j^u) = (1,0)$,
  \end{itemize}

  \noindent where $j^s$ and $j^u$ are the dimensions of the stable and unstable
  manifolds of $\mathbf{P}$ with respect to the reduced system, respectively.

  On the other hand, under WFH we also have the non-trivial eigenvalue
  $\lambda_2 = (f_i)_{\theta}(x_0, \theta_0, 0) \neq 0$ for the layer system
  and, therefore, the two possibilities:

  \begin{itemize}
    \item $\lambda_2 > 0 \Rightarrow (k^s, k^u) = (0,1)$; or
    \item $\lambda_2 < 0 \Rightarrow (k^s, k^u) = (1,0)$,
  \end{itemize}

  \noindent where $k^s$ and $k^u$ are the dimensions of the stable and unstable
  manifolds of $\mathbf{P}$ with respect to the layer system, respectively.

  Hence, observing that $j = \dim{\mathbf{P}} = 0$ and remembering
  \cref{sec:preliminaries:sub:gsp:thm:fenichel}, any combination of the signs of
  $\lambda_1$ and $\lambda_2$ leads to the total sum of dimensions

  \begin{equation*}
    (j^s + k^s) + (j^u + k^u) = 2 = \dim{S_i},
  \end{equation*}

  \noindent and, therefore, $\mathbf{P}$ acts as a hyperbolic singularity of
  $S_i$. Finally, the saddle-node duality comes from the fact that both
  non-trivial eigenvalues above have no imaginary parts.
\end{proof}

In other words, under WFH, the slow manifold $\mathcal{M}_i$ is, at minimum,
locally a graph. More than that, it is the entry-point for the external dynamics
to the cylinder. Besides that, it is normally hyperbolic at its full extend,
assuring then not only persistence and well-behaved stability for its invariant
compact parts, but also that $\mathcal{M}_i$ is always attracting or repelling
the surrounding (layer) dynamics. All these nice properties come at the low cost
of WFH. Therefore, it is not a surprise that, for every system studied below, we
require at least WFH, but also always test for SFH, whose importance will become
clear when studying affine systems.


==> sec/framework/sub/regularization.tex <==
\subsection{Regularization}%
\label{sec:framework:sub:regularization}

The next step of the framework consists, as presented at
\cref{sec:preliminaries:sub:regularization}, in the Sotomayor-Teixeira
regularization of the half planes $\Sigma_{12}$, $\Sigma_{23}$, $\Sigma_{34}$
and $\Sigma_{14}$, see \cref{sec:framework:sub:blowup:fig:framework_process}.
Since this part of the dynamics is well established, it is not always necessary
nor sufficient. However, for completeness, we present here the calculations for
reference on future works involving the external (radial) dynamics.

For $ij = 14$ or $ij = 23$, since the switching manifold $\Sigma_{ij}$ is
locally given as a subset of the zeros set of the map $(x,y,z) \to z$, then the
regularization is given by

\begin{equation*}
  \mathbf{F}_{ij}^{\varepsilon} =
  \frac{\mathbf{F}_i + \mathbf{F}_j}{2} +
  \varphi\left(\frac{z}{\varepsilon}\right)
  \frac{\mathbf{F}_i - \mathbf{F}_j}{2},
\end{equation*}

\noindent where $\varphi:\mathbb{R} \to \mathbb{R}$ is a monotonous transition
function. Now, assuming that $\mathbf{F}_{ij}^{\varepsilon} = \left(f_{ij},
  g_{ij}, h_{ij}\right)$ and applying the blow-up $\phi_2:\mathbb{R}^2 \times
  [0,\pi] \times \mathbb{R}^+ \to \mathbb{R}^3 \times \mathbb{R}$ given by

\begin{equation*}
  \phi_2(x, y, \psi, \eta) = (x, y, \eta \cos{\psi}, \eta \sin{\psi}),
\end{equation*}

\noindent we get a slow-fast system whose \textbf{slow dynamics} is given by

\begin{equation}
  \label{sec:framework:sub:regularization:eq:slow}
  \left\{\begin{matrix*}[l]
    \dot{x} = f_{ij}\\
    \dot{y} = g_{ij}\\
    0 = h_{ij} \sin{\psi}
  \end{matrix*}\right.
\end{equation}

\noindent and the \textbf{fast dynamics} is given by

\begin{equation}
  \label{sec:framework:sub:regularization:eq:fast}
  \left\{\begin{matrix*}[l]
    x' = 0\\
    y' = 0\\
    \psi' = -h_{ij} \sin{\psi}
  \end{matrix*}\right.,
\end{equation}

\noindent where $f_{ij}$, $g_{ij}$ and $h_{ij}$ must be calculated at the point
$\phi_2(x,y,\psi,0)$.

As a result, according to~\cite{Teixeira2012} and as presented at
\cref{sec:preliminaries:sub:gsp}, we get that the Filippov dynamics over
$\Sigma_{ij}$ is equivalent to the slow-fast dynamics given by
\cref{sec:framework:sub:regularization:eq:slow,sec:framework:sub:regularization:eq:fast}.
Analogous results can be obtained for $ij = 12$ and $ij = 34$. Finally, the
analysis of the dynamics over each half plane $\Sigma_{ij}$ can then be carried
out as presented in \cref{sec:preliminaries:sub:gsp:exmp:regul_process}.

